"I Don't Use AI for Everything": Exploring Utility, Attitude, and Responsibility of AI-empowered Tools in Software Development

AI-empowered tools have emerged as a transformative force, fundamentally reshaping the software development industry and promising far-reaching impacts across diverse sectors. This study investigates the adoption, impact, and security considerations of AI-empowered tools in the software development process. Through semi-structured interviews with 19 software practitioners from diverse backgrounds, we explore three key aspects: the utility of AI tools, developers' attitudes towards them, and security and privacy responsibilities. Our findings reveal widespread adoption of AI tools across various stages of software development. Developers generally express positive attitudes towards AI, viewing it as an efficiency-enhancing assistant rather than a job replacement threat. However, they also recognized limitations in AI's ability to handle complex, unfamiliar, or highly specialized tasks in software development. Regarding security and privacy, we found varying levels of risk awareness among developers, with larger companies implementing more comprehensive risk management strategies. Our study provides insights into the current state of AI adoption in software development and offers recommendations for practitioners, organizations, AI providers, and regulatory bodies to effectively navigate the integration of AI in the software industry.

==> 4_Result.tex <==
\section{Results}

In this section, we describe the findings from 20 semi-structured interviews with software practitioner software development engineers with experience in using AI-empowered tools for software projects.

In this study, the counts should be understood as the number of interviewees who mentioned the specific topic at least once during their interview. 
Followed by previous qualitative interview studies~\cite{}, these counts are not necessarily indicative of the broader developer population. 
Instead, they are provided to offer a general sense of the distribution of codes and to emphasize particularly common or uncommon themes that emerged during the interviews.











 


==> Tables/Comparison_matrix.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{booktabs}
% \usepackage{multirow}
\begin{table}[h]
\resizebox{\textwidth}{!}{
\begin{tabular}{@{}cp{2.8cm}p{2.3cm}ccp{2.5cm}@{}}
\toprule
\multirow{2}{*}{Transcription Software} & \multicolumn{2}{c}{Performance test} & \multicolumn{3}{c}{Other Aspects} \\ \cmidrule(l){2-6} 
 & Identify keywords in dialogue & Identify only Keywords & Limitations & Costs for unlimitation & Whether to Show Speakers \\ \midrule
Zoom & 99.3\% & 92\% & \textbf{-} & - & \checkmark \\
Teams & 98\% & 92\% & - & - & \checkmark \\
TurboScirbe & 100\% & 94\% & \multicolumn{1}{l}{Max 3 daily, up to 30 min} & 20 USD/per month & \checkmark \\
Otter & 97.4\% & 88\% & 300 min per month & 16.99 USD/per month & \checkmark \\
Tecent Conference & 67.1\% & 69.8\% & 1GB for Cloud Recording & 98 CNY/per month & \checkmark \\ \bottomrule
\end{tabular}
}
\caption{Comparison Matrix between Transcribing Tools}
\label{tab:my-table}
\end{table}

==> Tables/Tasks.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
\begin{table*}[ht]
\resizebox{\textwidth}{!}{
\begin{tabular}{llllll}
\hline
\textbf{Task Type}                           & \multicolumn{3}{l}{\textbf{Specific Tasks}}              & \multicolumn{2}{c}{\textbf{Explanation}} \\ \hline
\multirow{4}{*}{Ideation}                    & \multicolumn{3}{l}{Provision}                       & \multicolumn{2}{l}{Generate more ideas.}                     \\
                                             & \multicolumn{3}{l}{Verification}                    & \multicolumn{2}{l}{Verify if others have had the same ideas.}                     \\
                                             & \multicolumn{3}{l}{Optimization}                    & \multicolumn{2}{l}{Refine their ideas.}                     \\
                                             & \multicolumn{3}{l}{Supplement}                      & \multicolumn{2}{l}{Compensate for the inadequacy of existing ideas.}                     \\ \hline
\multirow{5}{*}{Documentation}               & \multicolumn{3}{l}{Design}                      & \multicolumn{2}{l}{Design and write development documents.}                     \\
                                             & \multicolumn{3}{l}{Analysis}                    & \multicolumn{2}{l}{Understand the content of documents.}                     \\
                                             & \multicolumn{3}{l}{Generation}                  & \multicolumn{2}{l}{Generate most of the content of the document and then fine-tune it.}                     \\
                                             & \multicolumn{3}{l}{Extension}                   & \multicolumn{2}{l}{Extend initial words, fleshing them out to reach the desired word count.}                     \\
                                             & \multicolumn{3}{l}{Rephrasing}                  & \multicolumn{2}{l}{Rephrase documents by polishing the grammar to enhance the overall quality.}                     \\ \hline
\multirow{13}{*}{Coding}                     & \multicolumn{3}{l}{Writing}                              & \multicolumn{2}{l}{Write codes.}                     \\
                                             & \multicolumn{3}{l}{Review}                               & \multicolumn{2}{l}{Review the code to improve the code quality based on code standard.}                     \\
                                             & \multicolumn{3}{l}{Checking}                             & \multicolumn{2}{l}{Check if there are errors of the code}                     \\
                                             & \multicolumn{3}{l}{Debugging}                            & \multicolumn{2}{l}{Assist with debugging if there's a problem in the code.}                     \\
                                             & \multicolumn{3}{l}{Optimization}                         & \multicolumn{2}{l}{Optimize the code performance.}                     \\
                                             & \multicolumn{3}{l}{Streamline}                           & \multicolumn{2}{l}{Simplify the code.}                     \\
                                             & \multicolumn{3}{l}{Testing}                              & \multicolumn{2}{l}{Write test cases.}                     \\
                                             & \multicolumn{3}{l}{Completion}                           & \multicolumn{2}{l}{Complete code. e.g. plug-ins / IDEA-integrated AI tools such as GitHub Copilot.}                     \\
                                             & \multicolumn{3}{l}{Explaination}                         & \multicolumn{2}{l}{Generate explanation of provided codes}                     \\
                                             & \multicolumn{3}{l}{Comments}                             & \multicolumn{2}{l}{Users will use AI tools to write code comments.}                     \\
                                             & \multicolumn{3}{l}{Simplicity}                           & \multicolumn{2}{l}{Simplify the code}                     \\ \hline
\multirow{5}{*}{Copywriting}                 & \multicolumn{3}{l}{Grammar Polishing}                    & \multicolumn{2}{l}{Correct grammatical errors and improve the overall language quality.}                     \\
                                             & \multicolumn{3}{l}{Text Rephrasing}                      & \multicolumn{2}{l}{Reword existing text.}                     \\
                                             & \multicolumn{3}{l}{Meeting Summary}                      & \multicolumn{2}{l}{Condense meeting notes into concise summaries.}                     \\
                                             & \multicolumn{3}{l}{Translation}                          & \multicolumn{2}{l}{Translation works}                     \\
                                             & \multicolumn{3}{l}{Text Writing}                         & \multicolumn{2}{l}{Write text.}                     \\ \hline
\multirow{7}{*}{Game Design}                 & \multicolumn{3}{l}{Game Content}                         & \multicolumn{2}{l}{Design the content of the game.}                     \\
                                             & \multicolumn{3}{l}{Prototype Design}                     & \multicolumn{2}{l}{Design prototypes during the game planning process.}                     \\
                                             & \multicolumn{3}{l}{Prototype Generation}                 & \multicolumn{2}{l}{Quickly generate some creative designs in our mind.}                     \\
                                             & \multicolumn{3}{l}{NPC Behavior Modeling}                & \multicolumn{2}{l}{Develop intelligent behaviors in NPC characters.}                     \\
 & \multicolumn{3}{l}{Worldview Structuring}& \multicolumn{2}{l}{Outline and develop the overall setting, lore, and context of the game world.}\\
                                             & \multicolumn{3}{l}{NPC Intellgience Enhancement}         & \multicolumn{2}{l}{Make NPCs in the game more intelligence.}                     \\
                                             & \multicolumn{3}{l}{NPC Dialogue Variation}               & \multicolumn{2}{l}{Generate multiple variations of NPC dialogue.}                     \\
                                             & \multicolumn{3}{l}{NPC Dialogue Generation}              & \multicolumn{2}{l}{Assist in creating dialogue for NPCs.}                     \\ \hline
Planning                                     & \multicolumn{3}{l}{Supplement}                      & \multicolumn{2}{l}{Compensate for the inadequacy of existing plans.}                     \\ \hline
Repeat Task                                  & \multicolumn{3}{l}{Repeat code}                          & \multicolumn{2}{l}{Write code that similar to what have done ("repeated code").}                     \\ \hline
\multirow{5}{*}{Cloud Information Searching} & \multicolumn{3}{l}{AWS CloudFormation Templates}         & \multicolumn{2}{l}{Search cloud formation templates.}                     \\
                                             & \multicolumn{3}{l}{Cloud Templates Generation}           & \multicolumn{2}{l}{}                     \\
                                             & \multicolumn{3}{l}{Cloud Infrastructure}                 & \multicolumn{2}{l}{Ask questions about the overall cloud infrastructure.}                     \\
                                             & \multicolumn{3}{l}{Terraform Settings}                   & \multicolumn{2}{l}{Terraform Settings - Configuration Language | Terraform | HashiCorp Developer}                     \\
                                             & \multicolumn{3}{l}{AWS Services}                         & \multicolumn{2}{l}{Query the AWS service.}                     \\ \hline
\end{tabular}
}

\end{table*}

==> Tables/persona_interview.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{booktabs}
% \usepackage{multirow}
% \usepackage[table,xcdraw]{xcolor}
% Beamer presentation requires \usepackage{colortbl} instead of \usepackage[table,xcdraw]{xcolor}
\begin{table}[h]
\begin{tabular}{@{}cccccc@{}}
\toprule
 & \multicolumn{5}{c}{Interview} \\ \cmidrule(l){2-6} 
\multirow{-2}{*}{Alias} & Duration & Recruitment Channel & Conversation Channel & Language & Date \\ \midrule
P1 & 00:40:19 & Personal Connection & Zoom & Mandarin &  16/04/2024\\
\rowcolor[HTML]{EFEFEF} 
P2 & 00:25:27 & Personal Connection & Zoom & Mandarin &  17/04/2024\\
P3 & 00:31:10 & Personal Connection & Zoom & Mandarin &  19/04/2024\\
\rowcolor[HTML]{EFEFEF} 
P4 & 00:29:29 & Personal Connection & Zoom & Mandarin &  21/04/2024\\
P5 & 00:28:06 & Personal Connection & Zoom & Mandarin &  21/04/2024\\
\rowcolor[HTML]{EFEFEF} 
P6 & 00:36:00 & Personal Connection & Teams & Mandarin &  21/04/2024\\
P7 & 00:38:14 & Personal Connection & Zoom & Mandarin &  23/04/2024\\
\rowcolor[HTML]{EFEFEF} 
P8 & 00:32:04 & Personal Connection & Tencent Conference & Mandarin &  24/04/2024\\
P9 & 00:35:36 & Personal Connection & Zoom & Mandarin &  25/04/2024\\
\rowcolor[HTML]{EFEFEF} 
P10 &  00:47:34& Personal Connection & Zoom & Mandarin &  29/04/2024\\
P11 &  00:37:29& Personal Connection & Zoom & Mandarin &  30/04/2024\\
\rowcolor[HTML]{EFEFEF} 
P12 &  00:22:15& Personal Connection & Tencent Conference & Mandarin &  30/04/2024\\
P13 &  00:26:46& Personal Connection & Zoom & Mandarin &  30/04/2024\\
\rowcolor[HTML]{EFEFEF} 
P14 &  00:28:04& Personal Connection & Zoom & Mandarin &  01/05/2024\\
P15 &  00:28:10& Personal Connection & Zoom & Mandarin &  02/05/2024\\
\rowcolor[HTML]{EFEFEF} 
P16 &  00:46:26& Personal Connection & Zoom & English &  15/05/2024\\
P17 &  00:31:00& Personal Connection & Zoom & Mandarin &  06/08/2024\\
\rowcolor[HTML]{EFEFEF} 
P18 &  00:24:50& Personal Connection & Zoom & Mandarin &  07/08/2024\\
P19 &  00:26:30& Personal Connection & Zoom & Mandarin &  09/08/2024\\ \bottomrule
\end{tabular}
\caption{Overview of 19 Interviews}
\label{tab:my-table}
\end{table}
